Characterizing the aerosol atmosphere above the Observatorio del Roque de los Muchachos by analyzing seven years of data taken with an GaAsP HPD-readout, absolutely calibrated elastic LIDAR

We present a new elastic LIDAR concept, based on a bi-axially mounted Nd:YAG laser and a telescope with HPD readout, combined with fast FADC signal digitization and offline pulse analysis. The LIDAR return signals have been extensively quality checked and absolutely calibrated. We analyze seven years of quasi-continuous LIDAR data taken during those nights when the MAGIC telescopes were operating. Characterization of the nocturnal ground layer yields zenith and azimuth angle dependent aerosol extinction scale heights for clear nights. We derive aerosol transmission statistics for light emitted from various altitudes throughout the year and separated by seasons. We find further seasonal dependencies of cloud base and top altitudes, but none for the LIDAR ratios of clouds. Finally, the night sky background light is characterized using the LIDAR photon backgrounds. abstract.txt

==> otherdevices.tex <==
\section{Supplementary Environmental Monitoring Devices}

\subsection{The Infrared Pyrometer}

\mga{J\"urgen, could you introduce here more information about the Pyrometer, and particularly the formula (maybe supported with a plot) for the calculation of the "cloudiness"? }

\mga{If that's fine, I might add a plot showing the correlation between $T_{3,6,9km}$ and (1-Cloudiness/100).}

\mwi{I'm not sure this pyrometer section is needed. The only place where the pyrometer is referenced is the very end where some comparison is made. I think it would be enough to briefly introduce the device and the term cloudiness there. I have the formula and some explanation in the AtmoHEAD proceeding \cite{will:atmohead2016} which could be used.}

A pyrometer of type \textit{Heitronics KT19.82} with a field of view of 2\degree is mounted on the side of the MAGIC-I telescope and points to the same sky region as the telescope. The measurement is passive and does not disturb the telescope operations. The pyrometer data can be used to detect the presence of clouds; it measures the integral thermal radiation from the sky in its line of sight in the wavelength range from 8\,\textmu m to 14\,\textmu m. The presence of a cloud can be inferred, since a cloud is ``warmer'' than the cloudless sky. The ``cloudiness'' is a unitless value between 0 and 100 calculated using an empirically derived function of the sky temperature measured by the pyrometer, ambient temperature and relative humidity from the weather station, and the zenith angle of the pyrometer pointing direction \mga{would be nice to have a reference for this: I have only Martin Fuchs' diploma thesis, is this the correct (and only?) reference? }. The ``cloudiness'' parameter correlates roughly with integrated atmospheric transmission from high altitudes to ground. It has the advantage of being measured every few seconds, instead of once per 3--5 minutes as in the case with the LIDAR measurements.

\subsection{The All-Sky-Camera}

\mga{Not sure what to do with this subsection: as it is now, it does not deserve a subsection of its own, but maybe enhanced with more technical information and particularly an image of the kind visible to the operators it might well remain here. Martin, it's your choice, a thorough description of the ASC may also go into a separate paper.}

\mwi{we are not really using the star and cloud detection described in the next paragraph. I would drop this ASC section.}

An AllSky camera is installed on the roof of the MAGIC Counting House, close to the LIDAR and the weather station. The images can be used to identify regions of the sky where the presence of clouds would hinder data taking of the MAGIC telescopes. A full picture is taken every 2~minutes and then analyzed to extract information about star visibility. Comparing the found stars in the image and their magnitude with catalog values for position and brightness, patches of clear and cloudy sky are determined. The validation of this method is still pending, so the results of such analyses are not used in this paper.

